GRPE: Relative Positional Encoding for Graph Transformer

We propose a novel positional encoding for learning graph on Transformer architecture. Existing approaches either linearize a graph to encode absolute position in the sequence of nodes, or encode relative position with another node using bias terms. The former loses preciseness of relative position from linearization, while the latter loses a tight integration of node-edge and node-topology interaction. To overcome the weakness of the previous approaches, our method encodes a graph without linearization and considers both node-topology and node-edge interaction. We name our method Graph Relative Positional Encoding dedicated to graph representation learning. Experiments conducted on various graph datasets show that the proposed method outperforms previous approaches significantly. Our code is publicly available at https://github.com/lenscloth/GRPE.

==> section/introduce_v2.tex <==
\section{Introduction}
\label{sec:intro}


% % The average cost of drug discovery increases drastically in a last decade with declining success rate of developing new therapeutics.
% % % To lower the cost of drug precursors and protein biotherapeutics design, efficient large scale screening with deep neural network draw large attention.
% % To lower the cost of drug discovery especially in the phase of lead finding and lead optimization, large scale screening with deep neural network draw large attention.
% % By representing molecule in a form of graph, a graph neural network can be utilized on the screening by predicting important properties, \eg, drug-likeness, solubility or synthesizability.
% % Therefore, graph representation learning has become a key technique for drug discovery.

% The average cost of drug discovery has increased drastically in the last decade with a declining success rate of developing new therapeutics.
% % To lower the cost of drug discovery, especially in the phase of lead finding and lead optimization, large-scale screening with deep neural networks draws large attention.
% Large-scale screening with deep neural networks draws considerable attention to lower the cost of drug discovery, especially in the lead finding and lead optimization phase.
% By representing a molecule in a graph, a graph neural network can be utilized on the screening by predicting important properties, \eg, drug-likeness, solubility, or synthesizability.
% Therefore, graph representation learning has become a key technique for drug discovery.

% Transformer introduced by \cite{vaswani2017attention}, has been effective in various forms inputs such as image, natural language and audios.

% Recent works have shown that Transformer \cite{vaswani2017attention} is effective in various forms of inputs such as natural language, audio, and image.
% Certain neural networks have inductive bias to encode positional information of inputs, \eg, convolutional neural network, graph convolutional network, or LSTM.
% However, self-attention of Transformer does not inherit inductive bias, thus explicit representations of position of inputs is necessary.

% Transformer \cite{vaswani2017attention} requires explicit representations of the position of inputs since self-attention does not have an inductive bias that assumes the order or position of inputs.
% Transformer \cite{vaswani2017attention} requires explicit representations of the position of inputs since self-attention does not have an inductive bias that assumes the order or position of inputs.
% Erasing inductive bias of a neural network enables Transformer to view long-term interaction between inputs demonstrating architectural efficacy on various subjects with various forms of inputs, \eg natural language processing, audio processing, or computer vision.

Transformer introduced by \cite{vaswani2017attention}, has been effective in graph representation learning, overcoming inductive biases of graph convolutional networks by using self-attention. 
On the other hand, explicit representations of position in graph convolutional networks are lost, thus incorporating graph structure on the hidden representations of self-attention is a key challenge.

% Certain neural networks, such as graph convolutional neural network or LSTM, have an inductive bias on the position of inputs.
% However, Transformer does not assume the order or position of inputs enabling viewing long-term interaction between inputs.

% In general, absolute positional encoding is widely adopted to represent the absolute position of each input.
% For instance, each word in a s

% The positional encoding to represent the position of each node in a graph is a key challenge in designing a Transformer for graph.
Representing the position of each node in a graph is a key challenge in designing a Transformer for graph.
In the case of natural language processing or computer vision, each input has its absolute position, \eg, $n$-th order of word in a sentence or coordinates of a patch within a grid.
In general, an embedding vector corresponding to the input's absolute position is added to each input embedding before feeding to Transformer.
% For example, the original work \cite{vaswani2017attention} leverages sinusoidal positional encoding.
However, adopting this absolute positional encoding on graph is not trivial since nodes of a graph do not have absolute position since there is no order between nodes.
% Instead, we leverage relative relation between nodes to define position of each node, and propose relative positional encoding for learning graph on Transformer.
% Transformer introduced by \cite{vaswani2017attention}, has been effective in graph representation learning, overcoming inductive biases of graph convolutional networks by using self-attention. 
% On the other hand, explicit representations of position in graph convolutional networks are lost, thus incorporating graph structure on the hidden representations of self-attention is a key challenge.

Several works have been proposed to incorporate positional information of graph on Transformer, and we categorize existing works into two: (a) linearizing graph with graph Laplacian to encode the absolute position of each node~\citep{gt_dwivedi2020generalization,san_kreuzer2021rethinking} (b) encoding position relative to another node with bias terms~\citep{ying2021transformers}. 
The former loses precision of position due to linearization, while the latter loses a tight integration of node-edge and node-spatial information.
To overcome the weakness of the two, we propose a novel positional encoding for graph which considers both relative position and the interaction with node.

To avoid losing relative position due to the linearization, we introduce two sets of learnable positional encoding vectors.
The first is spatial encoding to represent spatial relation between nodes.
The second is edge encoding to represent connection between nodes.
Our method considers the interaction between node features and the two encoding vectors to integrate both node-spatial relation and node-edge information when building attention map.
With the two positional encodings, topology of a graph can be represented in Transformer 
 without sacrficing precision.
Furthermore, we leverage the two positional encodings to incorporate graph topology on the hidden representations of self-attention.
% To avoid losing relative position due to the linearization, we propose to adopt the relative positional encoding by \cite{shaw2018self}.
% Its efficacy has been verified in natural language processing, however, the efficacy is not yet studied in a graph.
% Since the original work is designed for 1D word sequences, we reformulate to incorporate graph-specific properties.
% To this end, 
% Our method considers the interaction between node features and the two encoding vectors to integrate both node-spatial relation and node-edge information.
We name our method for graph representation learning as \textbf{G}raph \textbf{R}elative \textbf{P}ositional \textbf{E}ncoding (GRPE).

We extensively conducted experiments to validate the efficacy of our proposed method on various tasks, \eg, graph classification, graph regression and node classification.
Models built with our relative positional encoding achieve state-of-the-art performance on various graph datasets, showing the efficacy of our proposed method.


%%%%%%%%%%%%%%%% front page figure %%%%%%%%%%%%%%%%
\begin{figure}[t]
\vspace{-1cm}
\centering\includegraphics[width=\linewidth]{resource/GRPE_teaser.pdf}
\caption{
Our proposed Graph Relative Positional Encoding (GRPE). 
% GSA is a variant of self-attention module of Transformer~\citep{vaswani2017attention} to learn graph representation.
% GSA learns graph representation by encoding graph structure on both scaled dot product attention map. and the hidden representation.
GRPE is a relative positional encoding method dedicated to learn graph representation.
}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> section/introduction_old.tex <==
\section{Introduction}
\label{sec:intro}


% % The average cost of drug discovery increases drastically in a last decade with declining success rate of developing new therapeutics.
% % % To lower the cost of drug precursors and protein biotherapeutics design, efficient large scale screening with deep neural network draw large attention.
% % To lower the cost of drug discovery especially in the phase of lead finding and lead optimization, large scale screening with deep neural network draw large attention.
% % By representing molecule in a form of graph, a graph neural network can be utilized on the screening by predicting important properties, \eg, drug-likeness, solubility or synthesizability.
% % Therefore, graph representation learning has become a key technique for drug discovery.

% The average cost of drug discovery has increased drastically in the last decade with a declining success rate of developing new therapeutics.
% % To lower the cost of drug discovery, especially in the phase of lead finding and lead optimization, large-scale screening with deep neural networks draws large attention.
% Large-scale screening with deep neural networks draws considerable attention to lower the cost of drug discovery, especially in the lead finding and lead optimization phase.
% By representing a molecule in a graph, a graph neural network can be utilized on the screening by predicting important properties, \eg, drug-likeness, solubility, or synthesizability.
% Therefore, graph representation learning has become a key technique for drug discovery.

% Transformer introduced by \cite{vaswani2017attention}, has been effective in various forms inputs such as image, natural language and audios.

% Recent works have shown that Transformer \cite{vaswani2017attention} is effective in various forms of inputs such as natural language, audio, and image.
% Certain neural networks have inductive bias to encode positional information of inputs, \eg, convolutional neural network, graph convolutional network, or LSTM.
% However, self-attention of Transformer does not inherit inductive bias, thus explicit representations of position of inputs is necessary.

Transformer \cite{vaswani2017attention} requires explicit representations of the position of inputs since self-attention does not have an inductive bias that assumes the order or position of inputs.
Erasing inductive bias of a neural network enables Transformer to view long-term interaction between inputs demonstrating architectural efficacy on various subjects with various forms of inputs, \eg natural language processing, audio processing, or computer vision.

% Certain neural networks, such as graph convolutional neural network or LSTM, have an inductive bias on the position of inputs.
% However, Transformer does not assume the order or position of inputs enabling viewing long-term interaction between inputs.

% In general, absolute positional encoding is widely adopted to represent the absolute position of each input.
% For instance, each word in a s

% The positional encoding to represent the position of each node in a graph is a key challenge in designing a Transformer for graph.
Representing the position of each node in a graph is a key challenge in designing a Transformer for graph.
In the case of natural language processing or computer vision, each input has its absolute position, \eg, $n$-th order of word in a sentence or coordinates of a patch within a grid.
In general, positional embedding corresponding to the input's absolute position is added to each input embedding before feeding to Transformer.
For example, the original work \cite{vaswani2017attention} leverages sinusoidal positional encoding.
However, nodes of a graph do not have absolute positions since there is no order between nodes.
% Node's position can be defined with relative relation with 

Transformer introduced by \cite{vaswani2017attention}, has been effective in graph representation learning, overcoming inductive biases of graph convolutional networks by using self-attention. 
On the other hand, explicit representations of position in graph convolutional networks are lost, thus incorporating graph structure on the hidden representations of self-attention is a key challenge.
We categorize existing works into two: (a) linearizing graph with graph Laplacian to encode the absolute position of each node~\citep{gt_dwivedi2020generalization,san_kreuzer2021rethinking} (b) encoding position relative to another node with bias terms~\citep{ying2021transformers}. 
The former loses preciseness of position due to linearization, while the latter loses a tight integration of node-edge and node-spatial information.
Ours can be interpreted as overcoming the weakness of the two, which considers both relative position and the interaction with node.

To avoid losing relative position due to the linearization, we propose to adopt the relative positional encoding by \cite{shaw2018self}.
Its efficacy has been verified in natural language processing, however, the efficacy is not yet studied in a graph.
Since the original work is designed for 1D word sequences, we reformulate to incorporate graph-specific properties.
To this end, we introduce two sets of learnable positional encoding vectors to represent spatial relation or edge between two nodes.
Our method considers the interaction between node features and the two encoding vectors to integrate both node-spatial relation and node-edge information.
We name our method for graph representation learning as \textbf{G}raph \textbf{R}elative \textbf{P}ositional \textbf{E}ncoding (GRPE).

We extensively conducted experiments to validate the efficacy of our proposed method on various tasks from graph classification to graph regression.
Models built with our relative positional encoding achieve state-of-the-art performance on various molecule property prediction datasets, showing the efficacy of our proposed method.


%%%%%%%%%%%%%%%% front page figure %%%%%%%%%%%%%%%%
\begin{figure}[t]
\vspace{-1cm}
\centering\includegraphics[width=\linewidth]{resource/GRPE_teaser.pdf}
\caption{
Our proposed Graph Relative Positional Encoding (GRPE). 
% GSA is a variant of self-attention module of Transformer~\citep{vaswani2017attention} to learn graph representation.
% GSA learns graph representation by encoding graph structure on both scaled dot product attention map. and the hidden representation.
GRPE is a relative positional encoding method dedicated to learn graph representation.
}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> table/ablation-cifar10.tex <==

\begin{table*}
\centering
\caption {Ablation study results on CIFAR10 graph classification dataset with various configuration. Checkmark indicates that the component is being used. The first row is the configuration where all components are not used, and it is identical to a plain Transformer model.} % cifar maxhop=3
\label{tab:cifar10-ablation}
\begin{tabular}{cccccccc}
\toprule
\multicolumn{3}{c}{Context-aware Attention}  &
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\multirow{2}{*}{\makecell{Graph-embedded Value}}}  & 
\multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\multirow{2}{*}{\makecell{MNIST \\ Test Acc}}} &
% \multicolumn{1}{c}{\multirow{2}{*}{\makecell{Cifar10 \\ Test Acc}}} &
\multicolumn{1}{c}{\multirow{2}{*}{\makecell{Test Acc (\%)}}}
\\ \cline{1-1} \cline{3-3} 

\multicolumn{1}{c}{$b^{\text{query-context}}$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$b^{\text{key-context}}$} &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{}  &  
\multicolumn{1}{c}{} & 
% \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{} \\ \hline

% None
\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{\bf{98.50}}} &
\multicolumn{1}{c}{69.57} \\

% query only
\multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{98.16}} &
\multicolumn{1}{c}{74.60} \\

% key only
\multicolumn{1}{c}{-} & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-} & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{98.13}} &
\multicolumn{1}{c}{74.52} \\

% value only
\multicolumn{1}{c}{-} & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-} & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{97.14}} &
\multicolumn{1}{c}{70.04} \\

% query-key
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{98.27}} &
% \multicolumn{1}{c}{74.01} \\ 
\multicolumn{1}{c}{75.43} \\ 

% query-value
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{98.09}} &
% \multicolumn{1}{c}{75.53} \\ 
\multicolumn{1}{c}{77.22} \\ 

% key-value
\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{97.83}} &
% \multicolumn{1}{c}{75.05} \\ 
\multicolumn{1}{c}{77.49} \\ 

% all
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} &  \multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
% \multicolumn{1}{c}{\woonggi{98.27}} &
\multicolumn{1}{c}{\bf{77.86}} \\ 
% \hline \hline \\
\bottomrule
\end{tabular}
\end{table*}

% mnist hop3 추가실험 진행



% \begin{table*}[t]
% \centering
% \caption {Ablation study results on PCQM4M-LSC dataset with different configuration.} 
% \label{tab:pcqm4m-lsc-ablation}
% \begin{tabular}{lllllllllllll}
% \toprule
% \multicolumn{5}{c}{Structural Relation Encodings}                                                                                   & \multicolumn{1}{c}{} & \multicolumn{5}{c}{Edge Encodings}                                                                                       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{2}{*}{Validate MAE}} \\ \cline{1-1} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} \cline{11-11}
% \multicolumn{1}{c}{Query} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Key} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Value} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Query} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Key} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Value} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                              \\ \hline

% \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.01} \\

% \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.01} \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> table/ablation1.tex <==

\begin{table*}
\centering
\caption {Ablation study results on Cifar10 graph classification dataset with different configuration.} 
\label{tab:pcqm4m-lsc-ablation}
\begin{tabular}{lllllllllll}
\toprule
\multicolumn{5}{c}{Context-aware attention}                                                                                   & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Graph encoded value}                                                                                       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{2}{*}{Test Acc}} \\ \cline{1-1} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c}{query-context} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{key-context} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{edge features} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{structure feature(?)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{edge features} &   \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                              \\ \hline

\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   &       \multicolumn{1}{c}{} & \multicolumn{1}{c}{\woonggi{67.47}} \\

\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   &       \multicolumn{1}{c}{} & \multicolumn{1}{c}{\woonggi{69.95}} \\


\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   &       \multicolumn{1}{c}{} & \multicolumn{1}{c}{\woonggi{72.33}} \\


\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   &       \multicolumn{1}{c}{} & \multicolumn{1}{c}{\woonggi{71.46}} \\


\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   &       \multicolumn{1}{c}{} & \multicolumn{1}{c}{\woonggi{72.10}} \\

\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\woonggi{73.20}} \\
\hline \hline \\
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$}   &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{\woonggi{72.79}} \\

\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-}   &  \multicolumn{1}{c}{} 
& \multicolumn{1}{c}{\woonggi{72.01}} \\

\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{$\checkmark$}   &  \multicolumn{1}{c}{} 
& \multicolumn{1}{c}{\woonggi{70.74}} \\

\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{$\checkmark$}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} &
\multicolumn{1}{c}{-}   &  \multicolumn{1}{c}{} 
& \multicolumn{1}{c}{\woonggi{69.26}} \\

\bottomrule
\end{tabular}
\end{table*}

% \begin{table*}[t]
% \centering
% \caption {Ablation study results on PCQM4M-LSC dataset with different configuration.} 
% \label{tab:pcqm4m-lsc-ablation}
% \begin{tabular}{lllllllllllll}
% \toprule
% \multicolumn{5}{c}{Structural Relation Encodings}                                                                                   & \multicolumn{1}{c}{} & \multicolumn{5}{c}{Edge Encodings}                                                                                       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{2}{*}{Validate MAE}} \\ \cline{1-1} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} \cline{11-11}
% \multicolumn{1}{c}{Query} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Key} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Value} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Query} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Key} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Value} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                              \\ \hline

% \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.01} \\

% \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.01} \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> table/ablation2.tex <==
\begin{table}
\centering
\caption {Ablation study results on sharing structure embedding and edge embedding for all layers. We report MAE on ZINC dataset. The lower the better.} 
\label{tab:ablation2}
\scalebox{0.9}{
\begin{tabular}{ccc}
\toprule
\multicolumn{1}{c|}{Is shared?} & \multicolumn{1}{c|}{\#Params} & MAE \\ \hline
\multicolumn{1}{c|}{yes}  & \multicolumn{1}{c|}{489k} & 
\multicolumn{1}{c}{\textbf{0.094}$\pm$ 0.002}\\
\multicolumn{1}{c|}{no}  & \multicolumn{1}{c|}{579k} & 
\multicolumn{1}{c}{0.101 $\pm$ 0.003} \\
  
\bottomrule
\end{tabular}}
\end{table}


==> table/ablation_vn.tex <==

% \begin{table}
% \caption{Effects of sharing spatial encoding and edge encoding for all layers. We report MAE on ZINC dataset. The lower the better.}
% \centering
% \begin{tabular}{ccc}
% \toprule
% \multicolumn{1}{c|}{Is shared?} & \multicolumn{1}{c|}{\#Params} & MAE \\ \hline
% \multicolumn{1}{c|}{yes}  & \multicolumn{1}{c|}{489k} & 
% \multicolumn{1}{c}{\textbf{0.094}$\pm$ 0.002}\\
% \multicolumn{1}{c|}{no}  & \multicolumn{1}{c|}{579k} & 
% \multicolumn{1}{c}{0.101 $\pm$ 0.003} \\
% \bottomrule
% \caption{Hello}
% \end{tabular}

% \vspace{1cm}
% \begin{tabular}{ccc}
% \toprule
% \multicolumn{1}{c|}{Is shared?} & \multicolumn{1}{c|}{\#Params} & MAE \\ \hline
% \multicolumn{1}{c|}{yes}  & \multicolumn{1}{c|}{489k} & 
% \multicolumn{1}{c}{\textbf{0.094}$\pm$ 0.002}\\
% \multicolumn{1}{c|}{no}  & \multicolumn{1}{c|}{579k} & 
% \multicolumn{1}{c}{0.101 $\pm$ 0.003} \\
% \bottomrule
% \end{tabular}

% \label{tab:abl_sharing}
% \end{table}

\begin{table}
    \caption{Effects of virtual node on GRPE.}
    \begin{subtable}{\linewidth}
        \caption{Results on ZINC dataset of graph regression task. The lower the better.}
        \centering
         \begin{tabular}{cc|c}
        \toprule     
        \multicolumn{2}{c|}{How to represent entire graph?} &  \\
        \multicolumn{1}{c}{Global average pooling} & \multicolumn{1}{c|}{Virtual node} & \multicolumn{1}{c}{MAE} \\
        \hline
        \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c|}{-} & - \\
        \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{$\checkmark$} & \textbf{0.094} $\pm$ 0.002 \\
        \bottomrule
        
        \end{tabular}
    \label{tab:abl_vn_zinc}
    \end{subtable}\par

    \vspace{0.5cm}
    \begin{subtable}{\linewidth}
        \centering
        \caption{Results on CLUSTER of node classification task. The higher the better.}
        \begin{tabular}{c|c}
            \toprule Is virtual node included? & Weighted Accuracy\\\midrule
            -  &  \\
            $\checkmark$ &   \\\bottomrule
        \end{tabular}
        \label{tab:abl_vn_cluster}
    \end{subtable}
\end{table}

==> table/cifar10.tex <==

\begin{table}[t]
\centering
\caption {Results on CIFAR10 graph classification accuracy. The higher the better. } 
\label{tab:cifar10}
\scalebox{0.9}{
\begin{tabular}{ccc}
\toprule
\multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{\#Params} & ACC (\%) \\ \hline
\multicolumn{1}{l|}{MoNet~\cite{monti2017geometric}}  & \multicolumn{1}{c|}{101k} & 
\multicolumn{1}{c}{54.66$\pm$0.52} \\

\multicolumn{1}{l|}{GIN~\cite{gin_xu2018powerful}}  & \multicolumn{1}{c|}{106k} & 
\multicolumn{1}{c}{55.26$\pm$1.53} \\

\multicolumn{1}{l|}{GCN~\cite{gcn_kipf2016semi}}  & \multicolumn{1}{c|}{101k} & 
\multicolumn{1}{c}{55.71$\pm$0.38} \\

\multicolumn{1}{l|}{3WLGNN~\cite{maron2019provably}} &\multicolumn{1}{c|}{109k} & 
\multicolumn{1}{c}{59.18$\pm$1.59} \\

\multicolumn{1}{l|}{GAT~\cite{velivckovic2017graph}}  & \multicolumn{1}{c|}{111k} & 
\multicolumn{1}{c}{64.22$\pm$0.46} \\

\multicolumn{1}{l|}{GraphSage~\cite{graphsage_hamilton2017inductive}}  & \multicolumn{1}{c|}{105k} & 
\multicolumn{1}{c}{65.77$\pm$0.31} \\

\multicolumn{1}{l|}{EGT~\cite{hussain2021edge}}  & \multicolumn{1}{c|}{$\sim$100k} & 
\multicolumn{1}{c}{67.00$\pm$0.62} \\

\multicolumn{1}{l|}{GatedGCN~\cite{gated_bresson2017residual}}  & \multicolumn{1}{c|}{104k} & 
\multicolumn{1}{c}{67.31$\pm$0.31} \\

\multicolumn{1}{l|}{PNA~\cite{pna_corso2020principal}}  & \multicolumn{1}{c|}{$\sim$100k} & 
\multicolumn{1}{c}{70.35$\pm$0.63} \\

\multicolumn{1}{l|}{DGN~\cite{gated_bresson2017residual}}  & \multicolumn{1}{c|}{$\sim$100k} & 
\multicolumn{1}{c}{\bf{72.84}$\pm$0.42} \\


% \multicolumn{1}{l|}{$\dagger$Graphormer-FLAG~\cite{ying2021transformers}}  & \multicolumn{1}{c|}{47.0M} & 
% \multicolumn{1}{c}{80.51\pm0.53} \\
\hline 
\multicolumn{1}{l|}{$\dagger$GSA-Tiny (Ours)} &\multicolumn{1}{c|}{106k} & 
\multicolumn{1}{c}{68.13$\pm$0.23} \\
\hline \hline

\multicolumn{1}{l|}{RingGNN~\cite{chen2019equivalence}} &\multicolumn{1}{c|}{505k} & 
\multicolumn{1}{c}{39.17$\pm$17.11} \\

\multicolumn{1}{l|}{3WLGNN~\cite{maron2019provably}} &\multicolumn{1}{c|}{503k} & 
\multicolumn{1}{c}{58.04$\pm$2.51} \\

\hline
\multicolumn{1}{l|}{$\dagger$GSA-Tiny2x (Ours)} &\multicolumn{1}{c|}{409k} & 
\multicolumn{1}{c}{70.05$\pm$0.24} \\
\multicolumn{1}{l|}{$\dagger$GSA-Standard (Ours)} &\multicolumn{1}{c|}{46.2M} & 
\multicolumn{1}{c}{\bf{77.78$\pm$0.07}} \\
\bottomrule
\end{tabular}}
\end{table}


==> table/mnist.tex <==

\begin{table}[t]
\centering
\caption {Results on MNIST graph classification accuracy. The higher the better.} 
\label{tab:mnist}
\scalebox{0.9}{
\begin{tabular}{ccc}
\toprule
\multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{\#Params} & ACC (\%) \\ \hline

\multicolumn{1}{l|}{GCN~\cite{gcn_kipf2016semi}}  & \multicolumn{1}{c|}{101k} & 
\multicolumn{1}{c}{90.71$\pm$0.22} \\

\multicolumn{1}{l|}{MoNet~\cite{monti2017geometric}}  & \multicolumn{1}{c|}{104k} & 
\multicolumn{1}{c}{90.81$\pm$0.03} \\

\multicolumn{1}{l|}{3WLGNN~\cite{maron2019provably}} &\multicolumn{1}{c|}{108k} & 
\multicolumn{1}{c}{95.08$\pm$0.96} \\

\multicolumn{1}{l|}{GAT~\cite{velivckovic2017graph}}  & \multicolumn{1}{c|}{110k} & 
\multicolumn{1}{c}{ 95.54$\pm$0.21} \\

\multicolumn{1}{l|}{GIN~\cite{gin_xu2018powerful}}  & \multicolumn{1}{c|}{105k} & 
\multicolumn{1}{c}{96.49$\pm$0.25} \\

\multicolumn{1}{l|}{GraphSage~\cite{graphsage_hamilton2017inductive}}  & \multicolumn{1}{c|}{104k} & 
\multicolumn{1}{c}{97.31$\pm$0.10} \\

\multicolumn{1}{l|}{GatedGCN~\cite{gated_bresson2017residual}}  & \multicolumn{1}{c|}{104k} & 
\multicolumn{1}{c}{97.34$\pm$0.14} \\

\multicolumn{1}{l|}{EGT~\cite{hussain2021edge}}  & \multicolumn{1}{c|}{$\sim$100k} & 
\multicolumn{1}{c}{97.94$\pm$0.19} \\

\multicolumn{1}{l|}{PNA~\cite{pna_corso2020principal}}  & \multicolumn{1}{c|}{$\sim$100k} & 
\multicolumn{1}{c}{97.94$\pm$0.12} \\

\hline
% \multicolumn{1}{l|}{$\dagger$Graphormer-FLAG~\cite{ying2021transformers}}  & \multicolumn{1}{c|}{47.0M} & 
% \multicolumn{1}{c}{80.51\pm0.53} \\
\multicolumn{1}{l|}{$\dagger$GSA-Tiny (Ours)} &\multicolumn{1}{c|}{106k} & 
\multicolumn{1}{c}{ \bf{98.15 $\pm$ 0.14}} \\
\hline
\hline
\multicolumn{1}{l|}{RingGNN~\cite{chen2019equivalence}} &\multicolumn{1}{c|}{505k} & 
\multicolumn{1}{c}{91.86 $\pm$ 0.45} \\

\multicolumn{1}{l|}{3WLGNN~\cite{maron2019provably}} &\multicolumn{1}{c|}{502k} & 
\multicolumn{1}{c}{95.00 $\pm$ 0.42} \\

\hline
\multicolumn{1}{l|}{$\dagger$GSA-Tiny2x (Ours)} &\multicolumn{1}{c|}{409k} & 
\multicolumn{1}{c}{ \bf{98.20 $\pm$ 0.08}} \\

\multicolumn{1}{l|}{$\dagger$GSA-Standard(Ours)} &\multicolumn{1}{c|}{46.2M} & 
\multicolumn{1}{c}{ 98.18  $\pm$ 0.05} \\
\bottomrule
\end{tabular}}
\end{table}


